Quantum Natural Gradient with Efficient Backtracking Line Search

We consider the Quantum Natural Gradient Descent (QNGD) scheme which was recently proposed to train variational quantum algorithms. QNGD is Steepest Gradient Descent (SGD) operating on the complex projective space equipped with the Fubini-Study metric. Here we present an adaptive implementation of QNGD based on Armijo's rule, which is an efficient backtracking line search that enjoys a proven convergence. The proposed algorithm is tested using noisy simulators on three different models with various initializations. Our results show that Adaptive QNGD dynamically adapts the step size and consistently outperforms the original QNGD, which requires knowledge of optimal step size to {perform competitively}. In addition, we show that the additional complexity involved in performing the line search in Adaptive QNGD is minimal, ensuring the gains provided by the proposed adaptive strategy dominates any increase in complexity. Additionally, our benchmarking demonstrates that a simple SGD algorithm (implemented in the Euclidean space) equipped with the adaptive scheme above, can yield performances similar to the QNGD scheme with optimal step size. Our results are yet another confirmation of the importance of differential geometry in variational quantum computations. As a matter of fact, we foresee advanced mathematics to play a prominent role in the NISQ era in guiding the design of faster and more efficient algorithms.

==> junk.tex <==
% For this, an operator on the space of electronic wave functions is constructed suitable for evaluation on a quantum processor. This is achieved by first projecting the Hamiltonian onto a STO-3G basis set (a discrete basis set of molecular orbitals constituting a minimal set) \cite{hehre1972self}. This results in a fermionic Hamiltonian which is further mapped onto a two-qubit Hamiltonian \cite{o2016scalable,bravyi2017tapering,colless2018computation}, giving the following general form:
% \begin{align*}
    % H_{\mathrm{H}_2} = \alpha_0 I_1 I_2 + \alpha_1 Z_1I_2 + \alpha_2 I_1Z_2 + \alpha_3 Z_1Z_2 + \alpha_4 Y_1Y_2 + \alpha_5 X_1X_2,
% \end{align*}
% where $X_i, Y_i$ and $Z_i$ represent the Pauli operators acting on the $i$th qubits, and $\{\alpha_j \colon [0,5]\}$ are real valued coefficients which are a function of the inter-atomic distance between the two Hydrogen nuclie. 
% For the purpose of simulations, we consider two special cases of the Hamiltonian: \\
% (i) $ H_{\mathrm{H}_2}^{(1)}$ defined for the interatomic distance of at $0.735A$. Such a Hamiltonian has $\alpha_0 = -1.052373245772859$, $\alpha_1  = -\alpha_2 = -0.39793742484318045$,  $\alpha_3 =  -0.01128010425623538$, $\alpha_4 = 0$ and $\alpha_5 = 0.18093119978423156$, which has a minimum eigen value of ---.\\
% (ii) $H_{\mathrm{H}_2}^{(2)}$ (as simplified in \cite{bravyi2017tapering}) using $\alpha_0 = \alpha_3 = \alpha_4 = 0, \alpha_1  = \alpha_2 = 0.4, $ and $\alpha_5 = 0.2$ as
% For this, we use to different Hamiltonians to describe the energy quantization of the molecule. The first
% Ignoring the $ZZ$ 
% term, the Hamiltonian is given by 
